Beyond Individual and Group Fairness

We present a new data-driven model of fairness that, unlike existing static definitions of individual or group fairness is guided by the unfairness complaints received by the system. Our model supports multiple fairness criteria and takes into account their potential incompatibilities. We consider both a stochastic and an adversarial setting of our model. In the stochastic setting, we show that our framework can be naturally cast as a Markov Decision Process with stochastic losses, for which we give efficient vanishing regret algorithmic solutions. In the adversarial setting, we design efficient algorithms with competitive ratio guarantees. We also report the results of experiments with our algorithms and the stochastic framework on artificial datasets, to demonstrate their effectiveness empirically.

==> adversarial.tex <==
\section{Adversarial Setting}
\label{sec:adversarial}

In the previous section we studied a stochastic model for arrival of
complaints and designed no regret algorithms. In this section we study
the setting when we cannot make assumptions about the arrival of
complaints. In particular, we study an adversarial model where an
oblivious adversary chooses a sequence of complaints
$(i_1, \ell^{(i_1)}), (i_2, \ell^{(i_2)}), \dots, (i_t,
\ell^{(i_t)})$. For a given pair $(i, \ell^{(i)})$, index $i$
corresponds to the criterion $v_i$ in the graph $G$ to which the
complaint has been assigned, and $\ell^{(i)}$ is the non-negative loss
associated with the complaint. Similar to the setting from the
previous section, initially all the vertices in $G$ are in unfixed
state and each vertex has a fixing cost of $c_i$. At each time step
the algorithm can decide to fix a particular node. As a result all its
neighbors get unfixed. At time step $t$, if the criterion
corresponding to complaint $(i_t, \ell^{(i_t)})$ is fixed then the
algorithm incurs no loss. Otherwise, the algorithm incurs a loss of
$\ell^{(i_t)}$. The overall loss incurred by the algorithm is the
total fixing cost and the total loss incurred over the arrival
complaints. As before, we will denote a configuration of the vertices
in $G$ using a vector $s \in \{0,1\}^k$ with $s(i)=0$ representing an
unfixed vertex.  For an algorithm $\cA$ processing the request
sequence,
% let $y_{i,t}$ be a $\{0,1\}$ variable such that $y_{i,t}=1$ if
% vertex $i$ is unfixed at time step $t$. For a complaint $x_t$ let
% $i_t$ be the vertex in $G$ that the complaint is assigned
% to. Furthermore,
let $n_i$ be the total number of times vertex $v_i$ is fixed during
the course of the algorithm. The total loss of processing the
complaints is
\begin{align*}
    \text{Loss}(\cA) = \sum_{t=1}^T \ell^{(i_t)} \cdot \1(s_t(i_t) = 0) + \sum_{i=1}^k n_i c_i.
\end{align*}

Define $\OPT$ to be the algorithm that given the entire request
sequence in advance, makes the optimal choice of decisions to fix
vertices. Following standard terminology we define the
\emph{competitive ratio} of an algorithm $\cA$ to be the maximum of
$\text{Loss}(\cA)/\text{Loss}(\OPT)$ over all possible complaint
sequences. We will design efficient online algorithms for processing
the complaints that achieve a constant competitive ratio. Notice that
in this setting, in order for the competitive ratio to be finite, we
need to bound the range of the losses and the fixing costs of the
vertices. We will assume that the cost of fixing each vertex is at
least one and that the losses are bounded in the range $[0,R]$.

To get a better understanding of the above adversarial setting,
consider the case when the graph $G$ over the criteria has no edges,
i.e., there are no conflicts. In this case, given a sequence of
complaints, each with unit loss value, the optimal offline algorithm
that has the entire request sequence in advance can independently make
a decision for each vertex. In particular, if the total loss of the
complaints incurred at vertex $v_i$ exceeds the fixing cost $c_i$ then
the optimal decision is to fix the node $v_i$, and otherwise simply
incur the loss from the arriving complaints. In this case the online
algorithm can also simply process each vertex independently. At each
vertex the algorithm is faced with the classical \emph{ski-rental}
problem for which there exists a deterministic algorithm that is
$2$-competitive with optimal algorithm
\cite{karlin1988competitive}. For each vertex $i$, the online
algorithm simply waits till a total loss of $c_i$ or more has been
incurred on vertex $i$ and then decides to fix it. It is easy to see
that the total cost incurred by this strategy is at most twice the
cost incurred by \OPT.

However, the above algorithm will fail miserably in the presence of
conflicts in the graph $G$. As an example consider a graph with two
vertices $v_i$ and $v_j$ that are connected by an edge. Let the fixing
cost of $v_i$ be $1$ and the fixing cost of $v_j$ be $C \gg
1$. Consider a sequence of complaints, each of unit loss, consisting
of $C$ complaints for $v_j$ followed one complaint for $v_i$. If this
sequence is repeated $T$ times the optimal offline algorithm {\OPT}
incurs a loss of $C+T$ by fixing $v_j$ and incurring losses due to
$v_i$. However, the algorithm above will incur a cost of $(2C+2)T$
thereby leading to an unbounded competitive ratio. Hence, in order to
achieve a good competitive ratio one must make decisions not only
based on the loss incurred at the given vertex $v_i$, but also the
status of the vertices in the neighborhood of $v_i$. Our main result
in this section is the algorithm in Figure~\ref{ALG:adversarial} that
achieves a constant factor competitive ratio.

% Next, we consider the more challenging setting when the graph $G$ is
% an arbitrary graph.  In this case we first show in
% Theorem~\ref{thn:adversarial-opt} below that the optimal algorithm
% given a request sequence can be computed in polynomial time. The
% proof is provided in Appendix~\ref{sec:app-proofs-mdp}.
% \begin{theorem}
% \label{thm:adversarial-opt}
% Given a graph $G$ and a request sequence $x_1, x_2, \dots, x_T$,
% there is a polynomial time algorithm to compute the optimal sequence
% of decision to fix vertices, that results in the minimum total cost.
% \end{theorem}
% The algorithm above is based on a dynamic programming approach where
% the algorithm works backwards and decides the last vertex to be
% fixed in the sequence of decisions. After having made the particular
% choice, the problem reduces to finding the optimal sequence of fixes
% over a prefix of the requests.

\begin{figure}[t]
\begin{center}
\fbox{\parbox{1\textwidth}{
{\bf Input:} The graph $G$, fixing costs $c_i$, complaint sequence $(i_1, \ell^{(i_1)}),  \dots, (i_t, \ell^{(i_t)})$.
\begin{enumerate}   
\item For each $i \in [k]$, initialize $n^{(i)}, m^{(i)}$ to $0$.
\item Process the complaints in sequence and for each complaint $(i, \ell^{(i)})$ such that $v_i$ is unfixed do:
\begin{enumerate}
    \item $n^{(i)} = n^{(i)} + \ell^{(i)}$.
    \item If $n^{(i)} \geq \max \big( c_i, \sum_{j \in N(i)} m^{(j)}\big)$ fix $v_i$. Set $n^{(i)}$ to $0$ and $m^{(i)}$ to $c_i$. Set $m^{(j)} = 0$ for all $j \in N(i)$. 
    \item Otherwise, pick an arbitrary $j \in N(i)$ and set $m^{(j)} = \max(0, m^{(j)} - \ell^{(i)})$.
\end{enumerate}
\end{enumerate}
}}
\end{center}
\caption{\label{ALG:adversarial} Online algorithm for the adversarial setting.}
\end{figure}

The algorithm described in Figure~\ref{ALG:adversarial} makes
decisions based on local neighborhood information of a
vertex. Intuitively, if a vertex is fixed only once or a few times in
the optimal algorithm \OPT one would like to avoid fixing it too many
times. In order to achieve this, each time a vertex $v_i$ is fixed, it
adds a barrier of $m^{(i)} = c_i$ to the loss any of its neighbors
need to incur before getting fixed. Hence, if a vertex is connected to
a lot of fixed vertices then it has a high barrier to cross before
getting fixed. During the course of the algorithm each unfixed vertex
is in one of the two phases. In phase one, the vertex is accumulating
losses to pay for the barrier introduced by its neighbors (set (c) of
the algorithm). In phase two, once the barrier has been crossed the
vertex follows the standard ski-rental strategy independent of other
nodes for making a decision as to fix or not. The analysis becomes
delicate since a vertex may alternate between the two phases numerous
times. We next state the guarantee associated with our proposed
algorithm. The proof can be found in
Appendix~\ref{sec:app-proofs-mdp}.

\begin{theorem}
\label{thm:adversarial-online}
Given a graph $G$ with fixing costs at least one, the algorithm in Figure~\ref{ALG:adversarial} on any sequence of complaints with loss values in $[0,R]$ achieves a competitive ratio of at most $6R+2$.
\end{theorem}       


==> app.tex <==
% !TEX root=neurips.tex


\section{Proofs for the stochastic setting}
\label{sec:app-proofs-mdp}
We first show that in the stochastic model, if correlation sets are of size one then one can efficiently approximate the cost of the optimal state up to a factor of two.
\begin{reptheorem}{thm:opt-state-for-m-equal-1}
If correlations sets are of size one ($m = 1$), then, for any
$\e, \delta > 0$, the true parameter vector for $\MDP$ can be
approximated to $\e$-accuracy in $\ell_\infty$-norm with probability
at least $1 - \delta$, in at most
$O(\frac{\B^2 k}{\epsilon^2} \log (\frac{k}{\delta}))$ time steps and
exploring at most $k+1$ specific states in $\sS$. Furthermore, given a
parameter vector $\bm{\theta}$, there is an algorithm that runs in
time polynomial in $k$ and finds an approximately optimal state $s'$
such that $g(s') \leq 2 \min_{s \in \sS} g(s)$.
 \end{reptheorem}
\begin{proof}
Notice that when correlation sets are of size one, the expected loss incurred for criterion $v_i$ at any given state $s$ solely depends on whether $s(i)=0$ or $s(i)=1$. Hence in this case the MDP consists of $2k$ parameters where we use $\gamma^1_{i}$ and $\gamma^0_i$ to denote the expected losses incurred by vertex $i$ when it is in fixed and unfixed position respectively. For any $\delta > 0$, by Hoeffding's inequality, we have that if we stay in state $s = (0,0, \dots, 0)$ for $N = \frac{B^2}{\epsilon^2} \log(2k/\delta)$ time steps then with probability at least $1-\frac{\delta}{2}$, we have each $\gamma^0_i$ estimated up to $\epsilon$ accuracy. Let $e_i \in \{0,1\}^k$ denote the indicator vector for $i$. If we stay in state $s = e_i$ for $\frac{B^2}{\epsilon^2} \log(2k/\delta)$ time steps, then with probability at least $1-\frac{\delta}{2}$ we have $\gamma^1_i$ estimated up to $\epsilon$ accuracy. Hence, overall after $O(\frac{B^2 k}{\epsilon^2} \log (\frac{k}{\delta}))$ time steps, we have each parameter estimated up to $\epsilon$ accuracy. Notice that in total we observe at most $k+1$ states.


Next we show how to efficiently approximate the loss of the best state. Given the parameters of the MDP each vertex has two costs $\Lambda^{(1)}_i = \gamma^0_i$, denoting the cost incurred if the vertex is unfixed and
$\Lambda^{(2)}_i = c_i + \gamma^1_i$, denoting the cost incurred if the vertex is fixed. Without loss of generality assume that $\Lambda^{(1)}_i > \Lambda^{(2)}_i$~(any
vertex that does not satisfy this can be safely left unfixed). For each $i$, define $y_i=1$ if vertex $i$ is
unfixed otherwise define $y_i=0$. Then the offline problem of finding the best state can be written as 
\begin{align*}
    \text{min} & \sum_{i=1}^k (1-y_i) \Lambda^2_i + y_i\Lambda^1_i = \sum_{i=1}^k y_i \gamma_i + \sum_{i=1}^k \Lambda^{(2)}_i\\
    \text{s.t. } & y_i \in \{0,1\}\\
    y_i + y_j &\geq 1, \,\, \forall (v_i,v_j) \in E.
\end{align*}
Here $\gamma_i = \Lambda^{(1)}_i - \Lambda^{(2)}_i > 0$. By relaxing $y_i$ to be in
$[0,1]$ and solving the corresponding linear programming relaxation, we get a solution $y^*_1,
y^*_2, \dots, y^*_k$. Let $\text{LPval}$ denote the linear programming objective value achieved by $y^*_1,
y^*_2, \dots, y^*_k$. Since the linear programming formulation is a valid relaxation of the problem of finding the best state, we have $\text{LPval} \leq \min_{s \in \sS} g(s)$.

We output the state $s'$ in which a vertex $i$ if and only if $y^*_i <
1/2$. Let $S$ be the set of fixed vertices. We have
\begin{align*}
    g(s') &= \sum_{i \in S} \Lambda^{(2)}_i + \sum_{i \notin S} \Lambda^{(1)}_i\\
    &= \sum_{i=1}^k \Lambda^{(2)}_i + \sum_{i \notin S} (\Lambda^{(1)}_i - \Lambda^{(2)}_i)\\
    &= \sum_{i=1}^k \Lambda^{(2)}_i + \sum_{i \notin S} \gamma_i\\
    &< \sum_{i=1}^k \Lambda^{(2)}_i + 2\sum_{i \notin S} y^*_i\gamma_i\\
    &< 2 \Big(\sum_{i=1}^k \Lambda^{(2)}_i + \sum_{i=1}^k y^*_i\gamma_i \Big)\\
    &< 2 \cdot \text{LPval}\\
    &\leq \min_{s \in \sS} 2 g_{\bm{p}}(s).
\end{align*}
\end{proof}

We now show how to accurately estimate loss values for an arbitrary state of the MDP from loss values of a cover $\Phi$ of $\cC$ for the case of $m=2$. Recall that for any valid dichotomy $(i,j,b)$ we define $X^{i,j}_b$ as $X^{i,j}_b \coloneqq \mu_i^s - \mu_i^{s'}$,
where $s,s' \in \sK$ is an $(i,j,b)$ pair.

% \footnote{{\tt YM: what is $\ell^{(i)}$ and how it differes from $\ell_i^s$? What is the difference between $\mu^s_i$ and $\E[\ell^{(i)}|s]$? }}

\begin{reptheorem}{thm:phi-cover-m-equal-2}
Let $\sK$ be a cover for $\calC$. 
% and let $s, s' \in \sK$ be an
% $(i, j, b)$-pair. Define $X^{i,j}_b$ as
% $X^{i,j}_b \coloneqq \mu_i^s - \mu_i^{s'}$.
% %\mu_i^{s'} - \mu_i^s.
Then, for any state $s \in \sS$ and any $i \in [k]$ with $s(i) = b$, we have:
\begin{align}
\label{eq:vertex-loss-comp-m-equal-2}
\mu_i^s  
& = \mu_i^{s''}  + \sum_{j = 1}^k 
X^{i,j}_{b} \left[ \1(s(j) = 1) \1(s''(j) = 0) - 
\1(s(j) = 0) \1(s''(j) = 1) \right],
\end{align}
where $s''$ is any state in $\sK$ with $s''(i) = b$.
\end{reptheorem}
\begin{proof}
Consider a correlation set $\{i,j\}$. The expected loss incurred by vertex $v_i$ or $v_j$ due to this set in any given state depends solely on the configuration of $v_i$ and $v_j$ in that state. Hence there are four parameters in the $\bm{\theta}$ vector corresponding to the correlation set $\{i,j\}$ and we denote them using $\gamma^{a,b}_{i,j}$, where $a,b \in \{0,1\}$.
Let $s, s'$ be an $(i,j,b)$ pair. When we switch from $s$ to $s'$ the only difference in the expected losses for vertex $i$ comes from the pair $(i,j)$. Hence we have
\begin{align*}
\mu^{s'}_i - \mu^s_i &= \gamma^{b,1}_{i,j} - \gamma^{b,0}_{i,j}
\coloneqq X^{i,j}_b.
\end{align*}
Hence, given the loss estimates for states in $\Phi$ we can estimate $X^{i,j}_b$ for each $i,j \in [k]$ and $b \in \{0,1\}$. Next, given an arbitrary state $s$ with $s(i)=b$ let $s'' \in \Phi$ such that $s''(i)=b$. We have
\begin{align*}
    \mu^s_i &= \mu^{s''}_i + \sum_{\substack{j: s(j)=0 \\ s''(j)=1}} (\gamma^{b,0}_{i,j} - \gamma^{b,1}_{i,j}) + \sum_{\substack{j: s(j)=1 \\ s''(j)=0}} (\gamma^{b,1}_{i,j} - \gamma^{b,0}_{i,j})\\
     &= \mu^{s''}_i + \sum_{\substack{j:s(j)=1, \\ s''(j)=0}} X^{i,j}_{b}-\sum_{\substack{j:s(j)=0, \\ s''(j)=1}} X^{i,j}_{b}\\
    &= \mu_i^{s''}  + \sum_{j = 1}^k 
X^{i,j}_{b} \left[ \1(s(j) = 1) \1(s''(j) = 0) - 
\1(s(j) = 0) \1(s''(j) = 1) \right].
\end{align*}
\end{proof}
Next, we use the above theorem to establish the regret guarantee of the Algorithm in Figure~\ref{ALG:stochastic-mdp} for the case of $m=2$.
\begin{reptheorem}{thm:regred-mdp-m-equal-2}
Consider an $\MDP$ with losses in $[0, \B]$, a maximum fixing cost
$\cmax$, and correlations sets of size at most $m = 2$.  Let $\sK$ be
a cover of $\cC$ of size $r \leq 4k^2$, then, the algorithm of
Figure~\ref{ALG:stochastic-mdp} achieves a pseudo-regret bounded by
$O(k r^{1/3} (\cmax +\B) (\log rkT)^{1/3} T^{2/3})$. Furthermore,
given access to the optimization oracle for \eqref{eq:opt-state}, the
algorithm runs in time polynomial in $k$ and $n = |\cC|$.
\end{reptheorem}
\begin{proof}
In each time step the maximum loss incurred by any criterion is bounded by $c+B$. Let $\{s_1, s_2, \dots, s_r\}$ be the states in $\sK$. During the exploration phase the algorithm stays in each state for $N$ time steps and incurs a total loss bounded by $kNr (c+B)$. During the exploration phase the algorithm moves from one state to another in at most $k$ steps and incurs a total additional loss of at most $rk^2(c+B)$. At any given state $s \in \sK$ and vertex $v_i$, after $N$ time steps we will, with probability at least $1-\delta$, an estimate of $\mu^s_i$ up to an accuracy of $2B\sqrt{\frac{\log 1/\delta}{N}}$. Setting $\delta = 1/(rk T^4)$ and using union bound, we have that at the end of the exploration phase, with probability at least $1 - \frac{1}{T^4}$, the algorithm will have estimate $\hat{\mu}^s_i$ for all $s \in \sK$ and $i \in [k]$ such that
\begin{align}
\hat{\mu}^s_i - \mu^s_i \leq 4B\sqrt{\frac{\log rkT}{N}}.
\end{align}

% $$
% \Big| \hat{\E}[\ell^{(i)} | s] - {\E}[\ell^{(i)} | s] \Big| \leq 4R\sqrt{\frac{\log rkT}{N}}.
% $$
Hence during the exploitation phase, with high probability, the algorithm will have the estimate for the expected loss of each state in $\sS$, i.e., $\sum_i \mu^s_i$ up to an error of $4kB \sqrt{\frac{\log rkT}{N}}$. Combining the above we get that the total pseudo-regret of the algorithm is bounded by
\begin{align*}
 \Reg(\cA) &\leq  kNr(c+B) + rk^2 (c+B) + \Big(1-\frac{1}{T^4} \Big)4kB T \sqrt{\frac{\log rkT}{N}} + \frac{1}{T^4}k(c + B)T.
\end{align*}
Setting $N=10 \frac{T^{2/3}( \log rkT)^{1/3}}{r^{2/3}}$ we get that 
$$
\Reg(\cA) \leq O(k r^{1/3} (c+B) (\log rkT)^{1/3} T^{2/3}).
$$
\end{proof}

Having handled the case of $m=2$, we now generalize to higher $m$ by showing how to estimate the loss values at any state given the loss values for the states in a cover. Our algorihthm for general $m$ is described below.
\begin{figure}[t]
\begin{center}
\fbox{\parbox{1\textwidth}{
{\bf Input:} The graph $\sG$, correlation sets $\calC$, fixing costs $c_i$.
\begin{enumerate}   
\item Pick a cover $\sK =  \set{s_1, s_2, \dots, s_r}$ of $\cC$. 

\item Let $N=10 \frac{T^{2/3}( \log rkT)^{1/3}}{r^{2/3}}$.

\item For each state $s \in \sK$ do:

\begin{itemize}

\item Move from current state to $s$ in at most $k$ time steps.

\item Play action $a=0$ in state $s$ for the next $N$ time steps to
  obtain an estimate $\h \mu_i^s$ for all $i \in [k]$.

\end{itemize}

\item Using the estimated losses for the states in $\sK$ and
  Equation~\eqref{eq:vertex-loss-comp-m-general-app}, 
  %in Appendix~\ref{sec:app-proofs-mdp}, 
  run the oracle for the optimization \eqref{eq:opt-state} to obtain an approximately optimal state $\hat{s}$.
\item Move from current state to $\hat{s}$ and play action $a=0$ from $\hat{s}$ for the remaining time steps.
\end{enumerate}
}}
\end{center}
\caption{Online algorithm for general $m$ achieving $\tilde{O}(T^{2/3})$ pseudo-regret.}
\label{ALG:stochastic-mdp-general} 
\end{figure}

Recall that for a valid dichotomy $(i,b,J,u_1, u_2)$, we define $X^{i,u_1, u_2}_{b,J}$ as
\begin{align}
    \label{eq:def-x-general-m}
    X^{i,u_1, u_2}_{b,J} \coloneqq \mu^s_i - \mu^{s'}_{i},
\end{align}
where $s,s' \in \sK$ is an $(i,b,J,u_1, u_2)$ pair.

% \footnote{{\tt YM: Again, there is no definition of $X^{i, s_{-i}}_{b}$}}
\begin{reptheorem}{thm:phi-cover-m-general}
Let $\sK$ be a cover for $\calC$.
% and let $s,s' \in \sK$ be an $(i,b,J,u_1, u_2)$ pair. Define $X^{i,u_1, u_2}_{b,J} \coloneqq \mu^s_i - \mu^{s'}_{i}$. 
Then, for any state $s \in \sS$ and any $i \in [k]$ with $s(i) = b$, we have:
\begin{align}
% \label{eq:vertex-loss-comp-m-general}
%   \mu_i^s & = \mu_i^{s'} +  X^{i, s_{-i}}_{b} - X^{i, s'_{-i}}_{b},
% \end{align}
\label{eq:vertex-loss-comp-m-general-app}
  \mu_i^s & = \mu_i^{s''} +  \sum_{J \in I_i} X^{i, s(J), s''(J)}_{b,J}
\end{align}
Here $s''$ is any state in $\sK$ with $s''(i)=b$. 
\end{reptheorem}
\begin{proof}
Let $s,s' \in \sK$ be an $(i,b,J, u_1, u_2)$ pair. When we move from state $s$ to $s'$, the only difference between the expected losses incurred by vertex $v_i$ comes from the configuration of the vertices in $J$. Hence there at at most $2^{|J|+1}$ distinct parameters governing the expected loss incurred by vertex $i$ in a given state $s$ due to the configuration of the vertices in $J$. Denoting these parameters by $\gamma^{b,s(J)}_{i,J}$ we have
\begin{align*}
    \mu^{s'}_i - \mu^s_i = \gamma^{b,s'(J)}_{i,J} - \gamma^{b,s(J)}_{i,J} \coloneqq  X^{i,s'(J), s(J)}_{b,J}.
\end{align*}
Given the loss values for the states in the cover $\sK$, we can estimate the quantities $X^{i,s(J), s''(J)}_{b,J}$.

Next, for an arbitrary state $s$ such that $s(i)=b$, let $s'' \in \sK$ be such that $s''(i)=b$. We have
\begin{align*}
    \mu^s_i &= \mu^{s''}_i + \sum_{J \in I_i} \gamma^{b,s(J)}_{i,J} - \gamma^{b,s''(J)}_{i,J}\\
    &= \sum_{J \in I_i} X^{i, s(J), s''(J)}_{b,J}.
\end{align*}
% Let $s,s' \in \Phi$ be an $(i,b,u_1, u_2)$ and for ease of notation let $C_1, C_2, \dots, C_t$ be the correlation sets that $i$ participates in. The loss incurred by vertex $v_i$, at any given state $s$ solely depends on the configuration of the vertices in $\cup_j C_j$. Hence, the parameters in $\bm{\theta}$ that affect the loss incurred by vertex $i$ in any state $s$ can be denoted by $\theta^{i,s_{-i}}_1, \dots \theta^{i,s_{-i}}_t$.\footnote{{\tt YM: What is the difference from the previous definition of $\theta^s_j$?}} Notice that there are at most $2^{mt+1}$ such parameters. When we move from $s$ to $s'$ the only difference in the expected loss incurred by vertex $i$ comes from the change in configuration of the vertices in $\cup_j C_j$. Hence we can write
% \begin{align*}
% \E[\ell^{(i)}|s] - \E[\ell^{(i)}|s'] &= \sum_{j=1}^t \theta^{i,s_{-i}}_j - \theta^{i,s'_{-i}}_j\\
% & \coloneqq X^{i,s_{-i}}_b - X^{i,s'_{-i}}_b.
% \end{align*}
% Since $\Phi$ is cover for $\cC$ we can estimate $X^{i,s_{-i}}_b - X^{i,s'_{-i}}_b$ for all configurations $s_{-i}$ and $s_{-i}$ by estimating expected loss values for states in the cover.
% \footnote{{\tt YM: Seems like $X^{i, s_{-i}}_{b}=\mu^s_i$ so really the ONLY thing tio show is how to recover the parameters using the cover. I did not find any hint. What am I missing?}}
%
% using     \label{eq:vertex-loss-comp-m-general-app} this lets us estimate the expected loss values for vertex $v_i$ in any other state.
\end{proof}

\subsection{Beyond $T^{2/3}$ regret}
In this section we analyze the improved $\tilde{O}(\sqrt{T})$-regret algorithm from Figure \ref{ALG:stochastic-mdp-m=1-ucb-main}.
\ignore{
In this section we show that when the correlations sets in $\cC$ are of size one, one can get $\tilde{O}(\sqrt{T})$ regret in time polynomial in the size of the graph. In this case, the parameter vector ${\bm \theta}$ can be described using $2k$ parameters. More specifically, we will denote $\theta^0_i$ to be the expected loss incurred by vertex $v_i$ when it is unfixed and $\theta^1_i$ to be the expected loss incurred by vertex $v_i$ when it is fixed.
% \footnote{{\tt YM: Seems like the definition of $\theta$ is a moving target. We start with $\theta^s_i$, then $\theta^{i,s_{-i}}_j$ and not $\theta^0_i$. Having a different $\theta$ notation in each section is very confusing.}} 
In this case the cover $\sK$ is of size $k+1$ and includes the all zero state, as well as $k$ states corresponding to the indicator vectors of the $k$ vertices. Our algorithm is similar to the UCB algorithm for multi armed bandits \cite{auer2002finite} and maintains optimistic estimates of the parameters. For every vertex $i$, we will denote by $n^0_{i,t}$ to be the total number of time steps up to and including $t$, where the vertex $v_i$ is in an unfixed position, and $n^1_{i,t}$ to be the total number of times steps during which vertex $v_i$ is in a fixed position. For a given $\delta \in (0,1)$, and letting $\hat{\theta}^b_{i,t}$ to be the empirical expected loss observed when vertex $v_i$ is in state $b$, where $b \in \{0,1\}$, 
}
Recall that for any vertex $v_i$ and $b \in \{0,1\}$ the algorithm maintains the following optimistic estimates at each time step $t$,
\begin{align}
    \label{eq:optimistic-estimates}
    \tilde{\gamma}^b_{i,t} = \hat{\gamma}^b_{i,t} - 10B\sqrt{\frac{\log (kT/\delta)}{\tau^b_{i,t}}}.
\end{align}
\ignore{
In order to minimize the loss incurred when moving from one state to the next (due to fixing of certain criteria), our algorithm will work in episodes. In each episode $h$, the algorithm uses the current optimistic estimates to query the optimization oracle and find the current best state $s$. The algorithm then stays in the state $s$ for a certain number of time steps before querying the oracle again. The number of time steps spent per state are chosen carefully to avoid paying the fixing costs too often. 

The algorithm is sketched below.
\begin{figure}[t]
\begin{center}
\fbox{\parbox{1\textwidth}{
{\bf Input:} The graph $\sG$, correlation sets $\calC$, fixing costs $c_i$.
\begin{enumerate}   
\item Let $\sK$ be the cover of size $k+1$ that includes the all zeros state and the states corresponding to indicator vectors of the $k$ vertices. 

\item Move to each state in the cover once and update the optimistic estimates according to \eqref{eq:optimistic-estimates}.

\item For episodes $h = 1,2, \dots$ do:

\begin{itemize}

\item Run the optimization oracle \eqref{eq:opt-state} with the optimistic estimates as in \eqref{eq:optimistic-estimates} to get a state $s$.

\item Move from current state to state $s$. Stay in state $s$ for $\tau_h$ time steps and update the corresponding estimates using \eqref{eq:optimistic-estimates}. Here $\tau_h = \min_i n^{s(i)}_{i,t_h}$ and $t_h$ is the total number of time steps before episode $h$ starts.
\end{itemize}


\end{enumerate}
}}
\end{center}
\caption{Online algorithm for $m = 1$.}
\label{ALG:stochastic-mdp-m=1-ucb} 
\end{figure}
}
We will prove the following regret guarantee.
\begin{reptheorem}{thm:regred-mdp-m-equal-1-ucb}
Consider an $\MDP$ with losses bounded in $[0, B]$ and maximum cost of
fixing a vertex being $c$. Given correlations sets $\cC$ of
size one, the algorithm of Figure~\ref{ALG:stochastic-mdp-m=1-ucb-main} achieves a
pseudo-regret bounded by
$O(k^2 (c + B)^{2} \sqrt{T} \log T)$. Furthermore,
given access to the optimization oracle for \eqref{eq:opt-state}, the
algorithm runs in time polynomial in $k$.
\end{reptheorem}
\begin{proof}
We first bound the total number of different states visited by the algorithm. Initially the algorithm visits $k+1$ states in the cover. After that, each time the optimization oracle returns a new state $s$, by the definition of $t(h)$, the number of time steps where some vertex is in a $0$ or $1$ position is doubled. Hence, at most $O(k \log T)$ calls are made to the optimization oracle. Noticing that one can move from one state to another in at most $k$ time steps, the total loss incurred during the switching of the states is bounded by $O(k^2 (c+B) \log T)$. 
% \footnote{{\tt YM: I do not see how you get $k^3$. You have $k\log T $ switches, and each costs at most $k(\Gamma+R)$}}

For $\epsilon >0$ to be chosen later, we consider the episodes where the algorithm plays a state $s$ with expected loss at most $\epsilon$ more than that of the best state $s^*$. The total expected regret accumulated in these {\em good} episodes is at most $\epsilon T$. We next bound the expected regret accumulated during the bad episodes. 

From Hoeffding's inequality we have that for any time $t$, with probability at least $1-\frac{\delta}{T^3}$, for all $i \in [k],b \in \{0,1\}$,
\begin{align}
    \label{eq:concentration-of-estimates}
    \tilde{\gamma}^b_{i,t} + 20B\sqrt{\frac{\log (kT/\delta)}{\tau^b_{i,t}}} \geq \gamma^b_i \geq \tilde{\gamma}^b_{i,t}.
\end{align}
Let $G$ be the good event that \eqref{eq:concentration-of-estimates} holds for all $t \in [1,T]$. Conditioned on $G$ we also have that for any state $s$ and vertex $i$
\begin{align}
\label{eq:bound-on-optimistics-loss-per-state}
\mu^s_i \geq \tilde{\mu}^{s}_i, 
\end{align}
% The above implies that conditioned iexpected loss of a given state of the sum of the expected losses of the parameters in ${\bm \theta}$, conditioned on the event above we also have that for any state $s$,
% \begin{align}
% \label{eq:bound-on-optimistics-loss-per-state}
% \E[\ell | s] \geq \tilde{\ell}(s), 
% \end{align}
where $\tilde{\mu}^{s}_i$ is the estimated loss using the optimistic estimates. We will bound the expected regret accumulated in the bad episodes conditioned on the event $G$ above.

In order to do this we define certain key quantities. Consider a particular trajectory $\mathcal{T}$ of $T$ time steps executed by the algorithm. Furthermore, let $\mathcal{T}$ be such that the good event in \eqref{eq:concentration-of-estimates} holds during the $T$ time steps. We associate the following random variables with the trajectory. Let $N_\epsilon$ be the total number of time steps spent in bad episodes. Furthermore, let $\Reg_\epsilon$ be the total accumulated regret during these time steps. Then it is easy to see that $\E[\Reg_\epsilon | G] > \epsilon N_\epsilon$. For each vertex $v_i$ and $b \in \{0,1\}$ we define $\tau_\epsilon(i,b)$ to be the total number of time steps that vertex $v_i$ spends in bad episodes in position $b$ and $\tau_\epsilon(i,b,t)$ to be the total number of time steps spent in bad episodes up to time step $t$. Notice that
% \footnote{{\tt YM: Are you missing a "2" due to the $b\in\{0,1\}$}}
\begin{align}
\label{eq:sum-of-n-eps}
    \sum_b \sum_i \tau_\epsilon(i,b) \leq 2k N_\epsilon.
\end{align}

 Consider a particular bad episode $h$ and let $s$ be the state returned by the optimization oracle during that episode. Then conditioned on the good event $G$, the total regret $\Reg_{h}$ accumulated during episode $h$ satisfies
%  \footnote{{\tt YM: What is $\theta^{s(i)}_{i,t_h}$ do you mean $\tilde{\theta}^{s(i)}_{i,t_h}$}}
 \begin{align*}
    \E[{\Reg}_{h}|\mathcal{T}] &= \sum_i \big(\mu^s_i - \mu^{s^*}_i \big) t(h)\\
    &\leq \sum_i \big(\mu^s_i - \tilde{{\mu}}^{s^*}_i \big) t(h) & \big(\text{from} \eqref{eq:bound-on-optimistics-loss-per-state}\big)\\
    &\leq \sum_i \big(\mu^s_i - \tilde{{\mu}}^{s}_i \big) t(h) & \big(\text{since $s$ is best state according to the optimistic losses} \big)\\
    &\leq \sum_{i} \big(\gamma^{s(i)}_{i} - \tilde{\gamma}^{s(i)}_{i,t_h} \big) t(h) \\
    &\leq \sum_i 20B \sqrt{\frac{\log (kT/\delta)}{\tau^b_{i,t_h}}} t(h). & \big(\text{from \eqref{eq:optimistic-estimates}} \big)
\end{align*}
In the above inequality, the expectation is taken over the loss distribution for each vertex during states visited in the trajectory $\mathcal{T}$.
% \begin{align*}
%     {\Reg}_{h} &= \big(\E[\ell | s] - \E[\ell | s^*] \big) \tau_h\\
%     &\leq \big(\E[\ell | s] - \tilde{\ell}(s^*) \big) \tau_h & \big(\text{from} \eqref{eq:bound-on-optimistics-loss-per-state}\big)\\
%     &\leq \big(\E[\ell | s] - \tilde{\ell}(s) \big) \tau_h & \big(\text{since $s$ is best state according to the optimistic losses} \big)\\
%     &\leq \sum_{i} \big(\theta^{s(i)}_{i} - \theta^{s(i)}_{i,t_h} \big) \tau_h \\
%     &\leq \sum_i 20R \sqrt{\frac{\log (kT/\delta)}{n^b_{i,t_h}}} \tau_h. & \big(\text{from \eqref{eq:optimistic-estimates}} \big)
% \end{align*}
% \footnote{{\tt YM: I do not understand the last inequality. $n^b_{i,t_h}$ is a random variable, so what it is doing here? Actually $\tilde{\ell}$ and $\tilde{\theta}$ are also random variables!}}

%Denoting by $n_\epsilon(i,b,t_h)$ to be the total number of time steps vertex $i$ spends in bad episodes in position $b$ up to time step $t_h$. 
Since $\tau^b_{i,t_h} \geq \tau_\epsilon(i,b,t_h)$ we have
% \footnote{{\tt YM: $n_\epsilon(i,b,t_h)$ is a random variable. Do you the expected total number of steps, or with high probability? I am gettiung confused in this proof.}} 
we have that
\begin{align*}
    \E[{\Reg}_{h} | \mathcal{T}] &\leq \sum_i 20B \sqrt{\frac{\log (kT/\delta)}{\tau_\epsilon(i,b,t_h)}} t(h).
\end{align*}
Summing over bad episodes, the total expected regret in bad episodes can be bounded by
\begin{align}
\label{eq:reg-intermediate}
    \E[{\Reg}_{\epsilon} | \mathcal{T}] &\leq \sum_i \sum_b \sum_{h: h \text{ is bad }} 20B \sqrt{\frac{\log (kT/\delta)}{\tau_\epsilon(i,b,t_h)}} t(h).
\end{align}
Notice that $\tau_\epsilon(i,b,t_h) = \sum_{h' < h: h' \text{ is bad}} t(h')$. Furthermore, we know that (\cite{jaksch2010near}) for any sequence $z_1, z_2, \dots, z_h$ of non-negative numbers such that $z_i \geq 1$,
\begin{align}
\label{eq:bounded-sequence}
   \sum_{i=1}^h \frac{z_i}{\sqrt{\sum_{j=1}^{i-1} z_j}} &\leq (1+\sqrt{2})\sqrt{\sum_{i=1}^h z_i}.
\end{align}
From \eqref{eq:bounded-sequence} we get:
\begin{align*}
    \sum_{h: h \text{ is bad }}  \frac{t(h)}{\sqrt{\tau_\epsilon(i,b,t_h)}} &\leq \sqrt{\tau_\epsilon(i,b)}. 
\end{align*}
Substituting into \eqref{eq:reg-intermediate} we get that
\begin{align*}
    \E[{\Reg}_{\epsilon} | \mathcal{T}] &\leq \sum_i \sum_b 20B \sqrt{{\log (kT/\delta)}} \sqrt{\tau_\epsilon(i,b)}.
\end{align*}
Using \eqref{eq:sum-of-n-eps} we have that the above expected regret is maximized when $\tau_\epsilon(i,b)$ are equal, thereby implying 
\begin{align*}
    \E[{\Reg}_{\epsilon}|\mathcal{T}] &\leq 20Bk \sqrt{{\log (kT/\delta)}} \sqrt{N_\epsilon}.
\end{align*}
Using the fact that $\E[\Reg_\epsilon | G] > \epsilon N_\epsilon$ we get that conditioned on $G$,
\begin{align*}
    N_\epsilon \leq \frac{400 B^2 k^2 \log(kT/\delta)}{\epsilon^2}.
\end{align*}
Combining trajectories $\mathcal{T}$ where the good event $G$ holds, we get that the total expected regret accumulated in the bad episodes satisfies
\begin{align*}
    \E[{\Reg}_{\epsilon}|G] &\leq 20Bk \sqrt{{\log (kT/\delta)}} \sqrt{N_\epsilon}\\
    &\leq 400B^2 k^2 \frac{\log(kT/\delta)}{\epsilon}.
\end{align*}
Combining the above with the total expected regret accumulated in the good episodes, the loss of moving to different states, and the probability of good event $G$ not holding, we get
\begin{align*}
    {\Reg}(\cA) &\leq 400B^2 k^2 \frac{\log(kT/\delta)}{\epsilon} + \epsilon T + \frac{k(c+B)}{T^3} + O(k^2 (c+B) \log T).
\end{align*}
Setting $\epsilon = \frac{1}{\sqrt{T}}$  and $\delta = \frac{1}{T^4}$, we have the final bound
\begin{align*}
    {\Reg}(\cA) &\leq O\big((c+B)^2 k^2  \sqrt{T} \log(T)\big).
\end{align*}
\end{proof}


\subsection{Extension to higher $m$}

The algorithm in Figure~\ref{ALG:stochastic-mdp-m=1-ucb-main} extends to the case of higher $m$ assuming that each vertex does not participate in too many correlation sets. We say that vertices $v_i$ and $v_j$ are correlated if they both appear together in some correlation set in $\cC$. If a vertex $v_i$ appears in at most $O(\log k)$\footnote{{\tt YM: why $\log k$ and not a parameter?}} correlation sets, then the total loss incurred by vertex $v_i$ in any state depends on the position of $v_i$ and every other vertex that it is correlated with. Hence the total loss incurred by vertex $v_i$ depends on an $O(m \log k)$ dimensional vector specifying the current state of the vertex $v_i$ and other vertices that $v_i$ is correlated with.
% \footnote{{\tt YM: you mean "other states", it is unclear which vector are you referring to. }}. 
For every configuration ${\bm b}$ of this vector, we associate with each vertex $v_i$, parameters $\gamma^{\bm b}_i$. Notice that there are at most $O(k^m)$ such parameters. Each parameter is in turn a sum of a subset of the parameters in ${\bm \theta}$. Notice that in this case the size of the cover $\sK$ is upper bounded by $O(k^{m+1})$. Our algorithm for higher $m$ is similar to the one for $m=1$, but instead maintains optimistic estimates of the parameters $\gamma^{\bm b}_i$ via
\begin{align}
    \label{eq:optimistic-estimates-higher-m}
    \tilde{\gamma}^{\bm b}_{i,t} = \hat{\gamma}^{\bm b}_{i,t} - 10B\sqrt{m\frac{\log (kT/\delta)}{\tau^{\bm b}_{i,t}}}.
\end{align}
Here $\tau^{\bm b}_{i,t}$ is the total time spent up to and including $t$ where the vertex $i$ and the vertices that it is correlated with are in configuration ${\bm b}$. Similarly, for a given state $s$, we will denote by ${\bm s}(i)$, the configuration of the vertex $i$ and the vertices that it is correlated with.
Our algorithm is sketched below
\begin{figure}[h]
\begin{center}
\fbox{\parbox{1\textwidth}{
{\bf Input:} The graph $\sG$, correlation sets $\calC$, fixing costs $c_i$.
\begin{enumerate}   
\item Let $\sK$ be the cover of size $O(k^{m+1})$. 

\item Move to each state in the cover once and update the optimistic estimates according to \eqref{eq:optimistic-estimates-higher-m}.

\item For episodes $h = 1,2, \dots$ do:

\begin{itemize}

\item Run the optimization oracle \eqref{eq:opt-state} with the optimistic estimates as in \eqref{eq:optimistic-estimates-higher-m} to get a state $s$.

\item Move from current state to state $s$. Stay in state $s$ for $t(h)$ time steps and update the corresponding estimates using \eqref{eq:optimistic-estimates-higher-m}. Here $t(h) = \min_i \tau^{{\bm s}(i)}_{i,t_h}$ and $t_h$ is the total number of time steps before episode $h$ starts.
\end{itemize}


\end{enumerate}
}}
\end{center}
\caption{Online algorithm for higher $m$.}
\label{ALG:stochastic-mdp-m=higher--ucb} 
\end{figure}

For the algorithm above we have the following guarantee
% \footnote{{\tt YM: Do you mean expected regret? high probability regret? I think it cannot be absolute, since you have confidence bounds.}}
\begin{reptheorem}{thm:regred-mdp-m-higher-ucb}
Consider an $\MDP$ with losses bounded in $[0,B]$ and maximum cost of
fixing a vertex being $c$. Given correlations sets $\cC$ of size at most $m$ such that each vertex participates in at most $O(\log k)$ sets, there is an algorithm that achieves a
pseudo-regret bounded by
$O(m k^{2m+2} (c+B)^{2} \sqrt{T} \log T)$. Furthermore,
given access to the optimization oracle for \eqref{eq:opt-state}, the
algorithm runs in time polynomial in $O(k^{m + 1})$.
\end{reptheorem}
% An important corollary of the above is the following\footnote{{\tt YM: Are you using the previous theorem with $m=2$? So you should get $k^6$. What does the constant degree buy you?}}
% \begin{corollary}
% \label{cor:degree-d-graph}
% If $\cG$ is a constant degree graph with correlation sets consisting of subsets of edges in $\cG$, then the algorithm in Figure~\ref{ALG:stochastic-mdp-m=higher--ucb} achieves a pseudo-regret bounded by
% $O(k^6 (R + \Lambda)^{2} \sqrt{T} \log T)$.
% \end{corollary}
\begin{proof}
The proof is very similar to the proof of Theorem~\ref{thm:regred-mdp-m-equal-1-ucb}. Since each time the optimization oracle is called the time spent in some configuration ${\bm s}(i)$ is doubled, we get that the total number of calls to the optimization oracle are bounded by $O(k^m \log T)$. Hence the total loss incurred during the exploration phase can be bounded by $O(k^m (c+B) \log T)$. Let $G$ be the good event that \eqref{eq:optimistic-estimates-higher-m} holds for all $t \in [1,T]$.

As before, the loss incurred during good episodes is bounded by $\epsilon T$. Define $\tau_\epsilon(i, {\bm b})$ to be the total time that vertex $i$ and vertices that it is correlated with spend in configuration ${\bm b}$ during bad episodes. Then analogous to \eqref{eq:sum-of-n-eps} we have
\begin{align*}
    \sum_{{\bm b}} \sum_i \tau_\epsilon(i, {\bm b}) &\leq O(k^m) N_\epsilon.
\end{align*}
For a trajectory $\mathcal{T}$ where the good event $G$ holds,
the total expected regret in bad episodes can be bounded as
% \footnote{{\tt YM: I think you are missing $\sum_b$ in (17). Again, there is a mismatch between expectation (expected regret) and the random variables $n_\epsilon(i,{\bm b},t_h)$ and $N_\epsilon$}}
\begin{align}
\label{eq:reg-intermediate-general}
    \E[{\Reg}_{\epsilon}|\mathcal{T}] &\leq \sum_i \sum_b \sum_{h: h \text{ is bad }} 20B \sqrt{m \frac{\log (kT/\delta)}{\tau_\epsilon(i,{\bm b},t_h)}} t(h)\\
    &\leq \sum_i \sum_{{\bm b}} 20B \sqrt{m \log(kT/\delta)} \sqrt{\tau_\epsilon(i, {\bm b})}\\
    &\leq O(B k^{m+1})\sqrt{m \log(kT/\delta)} \sqrt{N_\epsilon}.
\end{align}
Using the fact that $\E[\Reg_\epsilon | \mathcal{T}] > \epsilon N_\epsilon$ we get that for a trajectory where the event $G$ holds,
\begin{align*}
    N_\epsilon \leq \frac{O(R^2 k^{2m+2} m \log(kT/\delta))}{\epsilon^2}.
\end{align*}
Hence we get that conditioned on the good event $G$, the total expected regret accumulated in the bad episodes is at most
\begin{align*}
    \E[{\Reg}_{\epsilon}|G] &\leq  O \big(R^2 m k^{2m+2} \frac{\log(kT/\delta)}{\epsilon} \big).
\end{align*}

Combining the above with the total expected regret accumulated in the good episodes, the loss of moving to different states, and the probability of the event $G$ not holding we get
\begin{align*}
    {\Reg}(\cA) &\leq O\big(B^2 m k^{2m+2} \frac{\log(kT/\delta)}{\epsilon}\big) + \epsilon T + \frac{k(c+B)}{T^3} + O(k^m \log T).
\end{align*}
Setting $\epsilon = \frac{1}{\sqrt{T}}$  and $\delta = \frac{1}{T^4}$, we have the final bound
\begin{align*}
    {\Reg}(\cA) &\leq O\big((c+B)^2 m  k^{2m+2}  \sqrt{T} \log(T)\big).
\end{align*}
\end{proof}
\section{Proofs for Section~\ref{sec:adversarial}}
\label{sec:app-adversarial}
In this section we establish the guarantee on the competitive ratio that is achieved by our online algorithm (Figure~\ref{ALG:adversarial}) for the adversarial setting. Notice that our algorithm in Figure~\ref{ALG:adversarial} is designed for a setting where in each time step complaints arrive for a single vertex in $\sG$. If multiple vertices accumulate complaints in a time step, we can simply order them arbitrarily and run the algorithm on the new sequence. Let {\OPT} be the optimal offline algorithm according to the chosen ordering of the complaints. Let {\OPT}' be the optimal offline algorithm when processing multiple complaints per time step. Notice that for each time step, the loss of {\OPT} cannot be larger than that of {\OPT}' since any choice available to {\OPT}' is available to {\OPT} as well. Hence it is enough to design an algorithm that is competitive with {\OPT}. In particular, we will prove the following theorem.
\begin{reptheorem}{thm:adversarial-online}
  Let $\sG$ be a graph with fixing costs at least one. Then, the
  algorithm of Figure~\ref{ALG:adversarial} achieves a competitive
  ratio of at most $6\B + 2$ on any sequence of complaints with loss values
  in $[0, \B]$.
  \end{reptheorem}
\begin{proof}
During the course of the algorithm, each vertex $v_i$ goes through multiple stages of being {\em unfixed} and then going back to the {\em fixed} state. Let us assume that $v_i$ goes through $r$ such stages. During each stage, before it can be fixed again, $v_i$ either incurs a loss that corresponds to its own fixing cost $c_i$ (step 2(b) of the algorithm) or incurs a loss that is used to payoff the past loss of a neighbor set (step 2(c)
% \footnote{{\tt YM: There is no (3c) do you mean (2c)?}} of the algorithm). 
Let $\delta^r_{i \to j}$ be the loss incurred by vertex $v_i$ during stage $r$ that is charged to the past loss of vertex $v_j$.\footnote{{\tt YM: I have no idea what you mean here, and it is definitely not a "definition" what is the charging scheme, and where is it define? I probably missed it.}}
%
Then during stage $r$, the total loss incurred by vertex $v_i$ can be bounded by $c_i + B + \sum_{j \in N(i)} \delta^r_{i \to j}$.

Notice that at each time step, the set of vertices fixed by the optimal offline algorithm {\OPT} form an independent set. Let $I_1, I_2, \dots, I_t$ be the distinct independent sets used by {\OPT} during the course of the algorithm. We will bound the loss incurred by the algorithm for each vertex $v_i$ by bounding the loss incurred by $v_i$ when it was part of an independent set of {\OPT}, and the loss incurred when it was not a part of any independent set. We define $\ell_{\text{in}}(v_i)$ to be the total loss incurred by the algorithm when $v_i$ was part of an independent set used by {\OPT}, and $\ell_{\text{out}}(v_i)$ to be the total loss incurred when $v_i$ was not in any independent set of {\OPT}. We will establish that the loss incurred when part of an independent set of {\OPT} can be charged to the loss incurred when not in any independent set. In particular, we have
\begin{align}
\label{eq:bound-on-v-in}
    \sum_{i=1}^k \ell_{\text{in}}(v_i) \leq 2B \Big( \text{Loss}(\OPT) +  \sum_{i=1}^k \ell_{\text{out}}(v_i) \Big).
\end{align}
To see the above inequality, consider a particular sequence of time steps when the vertex $v_i$ enters an independent set $I$ of {\OPT} and leaves the independent set at the end of the sequence. Let $\ell_{\text{in}}(v_i;I)$ be the loss incurred by $v_i$ during this particular sequence of time steps.
If the algorithm fixes $v_i$ $m$ times during the sequence then we have
\begin{align*}
\ell_{\text{in}}(v_i;I) \leq m(c_i + B) + \sum_r \sum_{j \in N(i)} \delta^r_{i \to j}.
\end{align*}

Here, $r$ ranges over all {\em unfix} to {\em fix} stages in this sequence. Furthermore, each additional time that $v_i$ is fixed by the algorithm, its neighbors must have incurred a total loss of at least $c_i$. Hence we can write
\begin{align*}
\ell_{\text{in}}(v_i;I) \leq (c_i + B) + \sum_{r'} \sum_{j \in N(i)} \delta^{r'}_{j \to i} + B \cdot \sum_r \sum_{j \in N(i)} \delta^r_{i \to j}.
\end{align*}

The losses $\delta^{r'}_{j \to i}$ were incurred by neighbors of $v_i$ during the time vertex $v_i$ was in the independent set $I$. Due to the constraints of the graph, none of the neighbors were in $I$ during this time. Next, consider a loss $\delta^r_{i \to j}$ incurred by vertex $v_i$ for past mistakes of a neighbor $j$. Notice that each $\delta^r_{i \to j} \leq c_j$. If during those past mistakes of $c_j$, vertex $v_j$ was not in the independent set of {\OPT}, then the optimal algorithm must have incurred a loss of at least $\delta^r_{i \to j}$ for fixing $c_j$. Hence, we can either charge this loss uniquely to the loss incurred by $v_j$ when it was not in an independent set, or to the loss incurred by {\OPT}. Finally, notice that since $v_i$ enters $I$ during the sequence, {\OPT} incurs a loss of at least $c_i$. Hence we get that
\begin{align*}
    \ell_{\text{in}}(v_i;I) \leq (c_i + B) + \sum_{r'} \sum_{j \in N(i)} \delta^{r'}_{j \to i} + B \cdot \sum_r \sum_{j \in N(i)} \delta^r_{i \to j}.
\end{align*}

Summing up over all the losses over independent sets $I$ we get
\begin{align*}
    \sum_{i=1}^k \ell_{\text{in}}(v_i) \leq 2B \Big( \text{Loss}(\OPT) +  \sum_{i=1}^k \ell_{\text{out}}(v_i) \Big).
\end{align*}

Next we bound $\sum_{i=1}^k \ell_{\text{out}}(v_i)$. Consider a particular sequence during which vertex $v_i$ exists the independent set of {\OPT} and enters back again at the end of the sequence. During this time period, the algorithm fixes $v_i$ multiple times and let $\ell_1, \ell_2, \dots, \ell_m$ be the losses sequence corresponding to vertex $v_i$ during this time period. Then the cost that {\OPT} incurs is at least $\ell_1 + \ell_2 + \dots + \ell_m + c_i$, where the term $c_i$ accounts for the fixing cost of $c_i$ as it enters the independent set of {\OPT} again. During this sequence, the loss incurred by the algorithm can be upper bounded by $\ell_1 + c_i + \ell_2 + c_i  + \dots + c_i \ell_m + (c_i + B)$. Notice that each of $\ell_2, \ell_3, \dots, \ell_m$ is at least $c_i$ since otherwise the algorithm would not have fixed $v_i$. Hence we get that during this time period the loss incurred by $v_i$ is at most $R$ times the loss incurred by {\OPT}. This implies
\begin{align*}
    \sum_{i=1}^k \ell_{\text{out}}(v_i) &\leq 2\cdot \text{Loss}(\OPT).
\end{align*}

Combining the above with \eqref{eq:bound-on-v-in} we get that
\begin{align*}
\text{Loss}(\cA) &= \sum_{i=1}^k \ell_{\text{in}}(v_i) + \sum_{i=1}^k \ell_{\text{in}}(v_i)\\
&\leq 2B \cdot \text{Loss}(\OPT) + (2B+1) \sum_{i=1}^k \ell_{\text{in}}(v_i)\\
&\leq (6B+2) \text{Loss}(\OPT).
\end{align*}
\end{proof}

% digraph FSM {
% rankdir = LR;
% nodesep = ".25";
% noderank = ".2";
% node [penwidth=1.5 shape=circle]

% 0 [label = "[0, 0, 0]", shape = circle, fontsize = 14, width=.75, fixedsize = "true"]
% 0 -> 0 [label = "0/&lambda;(0, 0)"];
% 0 -> 1 [label = "1/&lambda;(0, 1)"];
% 0 -> 2 [label = "2/&lambda;(0, 2)"];
% 0 -> 3 [label = "3/&lambda;(0, 3)"];

% 1 [label = "[1, 0, 0]", shape = circle, fontsize = 14, width=.75, fixedsize = "True"]
% 1 -> 1 [label = "0/&lambda;(1, 1)"];
% 1 -> 2 [label = "2/&lambda;(1, 2)"];
% 1 -> 3 [label = "3/&lambda;(1, 3)"];

% 2 [label = "[0, 1, 0]", shape = circle, fontsize = 14, width=.75, fixedsize = "True"]
% 2 -> 2 [label = "0/&lambda;(2, 2)"];
% 2 -> 1 [label = "1/&lambda;(2, 1)"];
% 2 -> 3 [label = "3/&lambda;(2, 3)"];

% 3 [label = "[0, 0, 1]", shape = circle, fontsize = 14, width=.75, fixedsize = "True"]
% 3 -> 2 [label = "2/&lambda;(3, 2)"];
% 3 -> 1 [label = "1/&lambda;(3, 1)"];
% }


